Rattling in spatially discrete diffusion equations with hysteresis

The paper treats a reaction-diffusion equation with hysteretic nonlinearity on a one-dimensional lattice. It arises as a result of the spatial discretization of the corresponding continuous model with so-called nontransverse initial data and exhibits a propagating microstructure --- which we call {\em rattling} --- in the hysteretic component of the solution. We analyze this microstructure and determine the speed of its propagation depending on the parameters of hysteresis and the nontransversality coefficient in the initial data.

==> conclusion.tex <==
\section{Conclusion and discussion}\label{secDiscussionConclusion}

In this paper, we have analyzed a microstructure arising in the spatially discretized version~\eqref{eqDiscretePrototype} of the continuous reaction-diffusion equation~\eqref{eqRDE} with hysteretic right-hand side and nontransverse initial data. We have shown that if a sufficiently regular pattern occurs, then the proportion between the switching and nonswitching nodes is uniquely determined by the hysteresis values $h_1$ and $-h_2$ (see~\eqref{eqDiscretePattern}), while the propagation speed can be found analytically and does not depend on the hysteresis value $-h_{2}$. To conclude, we formulate some open problems and indicate ways of further research.

\medskip

{\bf 1D patterns on lattices and their continuous limits.} The first step should be a rigorous proof of the rattling phenomenon, without an a priori assumption on existence of {\em some} pattern. We believe that the ideas suggested in this paper combined with the induction method used in~\cite{GurTikhRattling1-0} for $h_2=0$ must work. At least one should be able to prove the property~\eqref{eqPeriodicPattern} (which implies~\eqref{eqDiscretePattern}) in the case of rational $h_2/h_1$.

The next step would be to study the limit $\varepsilon\to 0$ in~\eqref{eqDiscretePrototype}. 
Consider the function
$$
H(x,\tau;\varepsilon):=\cH(v_n(\cdot;\varepsilon))(\tau),\quad
x\in[\varepsilon n-\varepsilon/2,\varepsilon n + \varepsilon/2), \
n\in\bbZ,
$$
which is supposed to approximate the hysteresis
$\cH(v)(x,\tau)$ in~\eqref{eqRDE}.
%It is easy to see that it
Assuming the dynamics \eqref{eqDiscretePattern} and \eqref{eqTauAsymp} and taking into account rescaling~\eqref{eqRescale}, we see that $H(x, \tau; \ep)$
has no pointwise limit as $\varepsilon\to 0$, but converges
in a certain weak sense to the function $H(x,\tau)$ given by
$H(x,\tau)=0$ for $\tau>ax^2$ and $H(x,\tau)=h_1$ for $\tau<ax^2$.
We emphasize that $H(x,\tau)$ does not
depend on $h_2$ (because $a$ does not). On the other hand, if
$h_2 > 0$, the hysteresis  $\cH(v)(x,\tau)$
in~\eqref{eqRDE} cannot take value $0$ by definition, which
clarifies the essential difficulty with the well-posedness of the
original problem~\eqref{eqRDE}, \eqref{eqRDEInitCond} in the nontransverse case. To
overcome the non-wellposedness, one need to allow the intermediate
value $0$ for the hysteresis operator.

Such a re-definition of hysteresis is consistent with the behavior
of $v(x,\tau)$ (also observed numerically) in the following sense. 
numerics indicates that,
as $\varepsilon\to 0$, the function
$$
V(x,\tau;\varepsilon):=v_n(\tau;\varepsilon),\quad
 x\in[\varepsilon n-\varepsilon/2,\varepsilon n + \varepsilon/2),\ n\in\bbZ,
$$
approximates a smooth function $V(x,\tau)$, which satisfies
$V(x,\tau)=0$ for $\tau>ax^2$ due to~\eqref{eqTauAsymp}. In other words, $V(x,\tau)$ sticks to the
threshold  $0$ on the expanding interval
$x\in(-\sqrt{\tau/a},\sqrt{\tau/a})$. Actually, one can prove that the functions $V(x,\tau)$ and $H(x,\tau)$ satisfy the relations
$$
\begin{aligned}
V_\tau=V_{xx}+H(x,\tau),\quad \tau>0,\ x\in\bbR,\\
V|_{\tau=0}=-cx^2,\quad x\in\bbR.
\end{aligned}
$$
However, the rigorous passage to the limit $\varepsilon\to 0$, the case of general nontransverse initial data $varphi(x)=-cx^2+o(x^2)$, and the description of the rattling microstructure in the continuous model are open questions. The latter one can probably be addressed with the help of  Young measures. In connection with passing to the limit, we mention~\cite{HelmersHerrmannMMS13}, where a hysteretic behavior of forward-backward diffusion equations is analyzed via spatial discretization. 


\medskip 

{\bf Multi-dimensional patterns.}  Numerics indicates that the switching pattern always obeys a law similar to~\eqref{eqDiscretePattern}. Figure~\ref{figMultiDim} illustrates the switching pattern for a two-dimensional analog of~\eqref{eqDiscretePrototypeZ} with the initial data $\varphi(x)=-c(x_1^2+x_2^2)$.
\begin{figure}[ht]
{\ \hfill\epsfxsize100mm\epsfbox{2d_rattling.eps}\hfill\ }
\caption{A snapshot for a time moment $\tau>0$ of a
two-dimensional spatial profile of hysteresis taking values
$h_1>4c>0$ and $h_2=h_1 > 0$. The nontrasverse initial data is
given by $\varphi(x)=-c(x_1^2+x_2^2)$. Grey (black) squares or
hexagons correspond to the nodes that have (not) switched on the
time interval $[0,\tau]$. a) Discretization on the square lattice.
b) Discretization on the triangular lattice.} \label{figMultiDim}
\end{figure} 
The rigorous analysis of the dynamics on multi-dimensional lattices for nontransverse initial data is has not been performed yet. 


\medskip

{\bf Rattling in slow-fast systems.} Let us replace the discontinuous hysteresis by a bi-stable slow-fast system
\begin{equation}\label{eqPrototypeSlowFast}
 v_\tau  = v_{xx}+w,\qquad
 \delta w_\tau=f(v,w),
\end{equation}
where $\delta>0$ is a small parameter and the nullcline of $f(v,w)$
is $Z$- or $S$-shaped. Formally, system~\eqref{eqPrototypeSlowFast}
can be treated as another regularization of
system~\eqref{eqRDE}, \eqref{eqRDEInitCond}. In the case where the nullcline of
$f(v,w)$ is $S$-shaped, one should replace $h_1$ and $-h_2$ in the
definition of hysteresis $\cH(v)$ by appropriate functions $H_1(v)$
and $H_2(v)$, see Fig.~\ref{figSShapedf}.

Surprisingly, the rattling persists. As $\delta\to 0$, the spatial profiles of $v$ and $w$
in~\eqref{eqPrototypeSlowFast} behave similarly to
$V(x,\tau;\varepsilon)$ and $H(x,\tau;\varepsilon)$, respectively,
as $\ep \to 0$, see Fig.~\ref{figSlowFastPattern}, with the
exception that the profile of $w$ remains continuous and forms steep
transition layers between mildly sloping steps of width tending to
$0$ as $\delta \to 0$.
Interestingly, the time-scale separation parameter $\delta$
in~\eqref{eqPrototypeSlowFast} yields the same effect as the
grid-size parameter $\ep$ in~\eqref{eqDiscretePrototypeZ}. Such a phenomenon for slow-fast systems is completely unexplored. 

\noindent
\begin{minipage}{\linewidth}
      \centering
      \begin{minipage}{0.48\linewidth}
\begin{figure}[H]
{\ \hfill\epsfxsize78mm\epsfbox{s_shaped.eps}\hfill\ }  \caption{a) The nullcline of the $S$-shaped nonlinearity $f(v,w)$.
b) Hysteresis with nonconstant branches $H_1(v)$ and $H_2(v)$.} \label{figSShapedf}
\end{figure}
      \end{minipage}
      \hspace{0.01\linewidth}
      \begin{minipage}{0.48\linewidth}
\begin{figure}[H]
{\ \hfill\epsfxsize70mm\epsfbox{slow_fast_rattling.eps}\hfill\ }
\caption{Upper and lower graphs are spatial profiles of the solution
$w(x,\tau)$ and $v(x,\tau)$, respectively, for
problem~\eqref{eqPrototypeSlowFast} with initial data
$v|_{\tau=0}=-cx^2 + o(x^2)$, $w|_{\tau=0}=h_1$.} \label{figSlowFastPattern}
\end{figure}
      \end{minipage}
 \end{minipage}  


